Large Scale Generative Multimodal Attribute Extraction for E-commerce Attributes

E-commerce websites (e.g. Amazon) have a plethora of structured and unstructured information (text and images) present on the product pages. Sellers often either don't label or mislabel values of the attributes (e.g. color, size etc.) for their products. Automatically identifying these attribute values from an eCommerce product page that contains both text and images is a challenging task, especially when the attribute value is not explicitly mentioned in the catalog. In this paper, we present a scalable solution for this problem where we pose attribute extraction problem as a question-answering task, which we solve using \textbf{MXT}, consisting of three key components: (i) \textbf{M}AG (Multimodal Adaptation Gate), (ii) \textbf{X}ception network, and (iii) \textbf{T}5 encoder-decoder. Our system consists of a generative model that \emph{generates} attribute-values for a given product by using both textual and visual characteristics (e.g. images) of the product. We show that our system is capable of handling zero-shot attribute prediction (when attribute value is not seen in training data) and value-absent prediction (when attribute value is not mentioned in the text) which are missing in traditional classification-based and NER-based models respectively. We have trained our models using distant supervision, removing dependency on human labeling, thus making them practical for real-world applications. With this framework, we are able to train a single model for 1000s of (product-type, attribute) pairs, thus reducing the overhead of training and maintaining separate models. Extensive experiments on two real world datasets show that our framework improves the absolute recall@90P by 10.16\% and 6.9\% from the existing state of the art models. In a popular e-commerce store, we have deployed our models for 1000s of (product-type, attribute) pairs.

==> related.tex <==
\section{Related Work}
Early 2000's saw a tremendous growth in e-commerce business, leading to multiple works focusing on extracting attribute values from product pages.
\label{sec:related}
\vspace{-0.1in}
\subsection{Text Only Attribute Extraction Models}
Some of the early work started extracting attribute values from textual content of the products. Ghani et. al.~\cite{Ghani2006TextMF} 
solved this problem by using semi-supervised classification based algorithms to extract attribute values from textual product descriptions. 
Putthividhya and Hu~\cite{Putthividhya2011BootstrappedNE} proposed use of NER on short titles to extract attribute values using multiple base 
classifiers along with CRF layer. Recently, Open-tag model by Zheng et. al.~\cite{Zheng2018OpenTagOA} saw a tremendous success in attribute-value 
extraction problem where they used LSTM with CRF along with attention mechanism to extract attribute values from textual product descriptions. 
Then Mehta et. al.~\cite{Mehta2021LATEXNumericLA} proposed Latex, an NER-based model for extracting numeric attributes from product text. Some 
of the recent works~\cite{Wang2020LearningTE, Shrimal2022NERMQMRCFN} have solved the attribute extraction problem by posing the NER problem 
as a question-answering task and solving them using transformer-based models. Most of the above works have formulated the attribute extraction 
task as a sequence tagging problem, hence they can extract attribute only when the attribute-values are explicitly stated in the product text. 
The advantage of these methods is that they can extract the attribute values which are never seen during training.
\vspace{-0.1in}
\subsection{Multi-modal Attribute Extraction Models}
Recently, more attention has been given to predicting attribute values by utilizing the product images as well. Zhu et. al.~\cite{Zhu2020MultimodalJA}
proposed learning multi-modal hidden representations to solve the sequence-tagging task for attribute extraction. Again, this work formulates 
attribute extraction as a sequence-tagging problem. Recently, the CMA-CLIP model~\cite{Liu2021CMACLIPCA} posed the attribute extraction task 
as a multi-modal, multi-task, multi-class classification task where they have used CLIP~\cite{Radford2021LearningTV} for learning multi-modal 
embeddings, followed by applying two attention modules (sequence-wise and modality wise). Their model has an advantage that the attribute value 
needn't be present in the product text. However, classification-based models face a challenge that they can predict the attribute value from 
a pre-defined set of values. But since most of the attribute values keep on changing and hence picking them from a pre-defined set or tagging 
is inaccurate. In the generative based approach (where attribute-values are generated by the model), the benefit is that the model can produce 
the correct attribute value even if it is phrased differently in the input texts or even if it is not seen in the training data (as we will 
demonstrate in section~\ref{subsec:zero_shot}). 

There has been little work in generative based approaches for attribute extraction. The approach presented in the 
paper\cite{roy-etal-2021-attribute} formulates the attribute value extraction as an instance of text infilling task and 
an answer generation task. They utilize Infilling by Language Modeling (ILM) \cite{Donahue2020EnablingLM} for the infilling 
approach and they fine-tuned a Text-to-Text Transfer Transformer (T5)\cite{Raffel2020ExploringTL} on an answer generation task. 
% This approach does not work well for the use-case where the attribute value is to be inferred from image. 
PAM~\cite{Lin2021PAMUP} is a recent attribute-generation model that has shifted focus from unimodal attribute extraction to multi-modal. 
However, this model has the limitation to scale only for a few product categories, as during training, it requires creating separate 
pre-defined vocabularies for each product type and selecting output tokens from those vocabularies. Creating these vocabularies for each 
product type is not scalable. The results shown in the paper are for only two product types rather than for the diverse set of attributes 
and products.
